Mixed Precision Training With 8-bit Floating Point

Reduced precision computation for deep neural networks is one of the key areas addressing the widening compute gap driven by an exponential growth in model size. In recent years, deep learning training has largely migrated to 16-bit precision, with significant gains in performance and energy efficiency. However, attempts to train DNNs at 8-bit precision have met with significant challenges because of the higher precision and dynamic range requirements of back-propagation. In this paper, we propose a method to train deep neural networks using 8-bit floating point representation for weights, activations, errors, and gradients. In addition to reducing compute precision, we also reduced the precision requirements for the master copy of weights from 32-bit to 16-bit. We demonstrate state-of-the-art accuracy across multiple data sets (imagenet-1K, WMT16) and a broader set of workloads (Resnet-18/34/50, GNMT, Transformer) than previously reported. We propose an enhanced loss scaling method to augment the reduced subnormal range of 8-bit floating point for improved error propagation. We also examine the impact of quantization noise on generalization and propose a stochastic rounding technique to address gradient noise. As a result of applying all these techniques, we report slightly higher validation accuracy compared to full precision baseline.

==> discussion.tex <==
\section{Discussion}\label{discussion}
Our proposed solution is generalized widely applicable for the following reasons: 
\item We have simplified the hardware requirements by eliminating the need for stochastic rounding hardware in the critical compute path, as proposed in \cite{NIPS2018_fp8}, which makes our solution friendly to dense systolic array implementation. 
\item We have demonstrated the robustness of our training method with broad coverage across image recognition and machine translation workloads.   

Discuss why we did not pursue 16-bit accumulator -- cite progressive accumulation in systolic arrays to justify. Other reason is the additional cost involved with building chunk based accumulation (this maynot be that big) and stochastic rounding support inside the systolic array. Our solution can get higher compute density because we don't have to do this circus. 

Stochastic rounding cost during down conversion is minimal -- talk about how simple the 8-bit LFSR implementation is. Discuss random number sharing? 
